Sound Patch Generation for Vulnerabilities

Security vulnerabilities are among the most critical software defects in existence. As such, they require patches that are correct and quickly deployed. This motivates an automatic patch generation method that emphasizes both soundness and wide applicability. To address this challenge, we propose Senx, which uses three novel patch generation techniques to create patches for out-of-bounds read/write vulnerabilities. Senx uses symbolic execution to extract expressions from the source code of a target application to synthesize patches. To reduce the runtime overhead of patches, it uses loop cloning and access range analysis to analyze loops involved in these vulnerabilities and elevate patches outside of loops. For vulnerabilities that span multiple functions, Senx uses expression translation to translate expressions and place them in a function scope where all values are available to create the patch. This enables Senx to patch vulnerabilities with complex loops and interprocedural dependencies that previous semantics-based patch generation systems cannot handle. We have implemented a prototype using this approach. Our evaluation shows that the patches generated by Senx successfully fix 76% of 42 real-world vulnerabilities from 11 applications including various tools or libraries for manipulating graphics/media files, a programming language interpreter, a relational database engine, a collection of programming tools for creating and managing binary programs, and a collection of basic file, shell, and text manipulation tools. All patches that Senx produces are sound, and Senx correctly aborts patch generations in cases where its analysis will fall short.

==> macros.tex <==
\newcommand{\nmappings}{11314}
\newcommand{\napps}{1260}

%%%%% Figure -related commands

\renewcommand{\dbltopfraction}{1.0}
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.2}

%\renewcommand{\subfigtopskip}{0pt}
%\renewcommand{\subfigcapskip}{0pt}

%\newcommand{\mysubfig}[3]
%{
%\subfigure[#2]{
%\ifpdf
%\includegraphics[width=#3\linewidth]{#1}
%\else
%\includegraphics[width=#3\linewidth]{#1}
%\fi
%}
%}


\newcommand{\myfig}[5]
{
\begin{figure}[t]
\begin{center}
\ifpdf
\includegraphics[width=#4\linewidth]{#1}
\else
\includegraphics[width=#4\linewidth]{#1}
%\rotatebox{-90}{\includegraphics[width=0.8\linewidth]{#1}}
\fi
\end{center}
\vspace{#5}
\caption{#2}\label{#3}
%\vspace{-10pt}
\end{figure}
}

\newcommand{\myfigwide}[5]
{
\begin{figure*}[t]
%\vspace{-10pt}
\begin{center}
\ifpdf
\includegraphics[width=#4\linewidth]{#1}
\else
\includegraphics[width=#4\linewidth]{#1}
%\rotatebox{-90}{\includegraphics[width=#4\linewidth]{#1}}
\fi
\end{center}
\vspace{#5}
\caption{#2}\label{#3}
%\vspace{-10pt}
\end{figure*}
}

\newcommand{\mysubfigtwo}[8]
{
\begin{figure}
        \centering
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#1}
                \caption{#2}
                \label{#3}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#4}
                \caption{#5}
                \label{#6}
        \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \caption{#7}\label{#8}
        \vspace{-15pt}        
\end{figure}
}

\newcommand{\myfigthreevert}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\myfigthreevertcont
}

\newcommand{\myfigthreevertcont}[2]
{
\begin{figure}
        \centering
         \begin{tabular}{c}
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempa}
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
	\\
	\\
	~
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempd}
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}%
	\\
	\\
	~
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempg}
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}%
	\\
	\\
	\end{tabular}
	~
	\caption{#1}\label{#2}
        \vspace{-5pt}        
\end{figure}
}
\newcommand{\myfigthreevertbox}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\myfigthreevertboxcont
}

\newcommand{\myfigthreevertboxcont}[2]
{
\begin{figure}
        \centering
         \begin{tabular}{c}
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempa}}%
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
	\\
	\\
	~
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempd}}%
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}%
	\\
	\\
	~
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempg}}%
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}%
	\\
	\\
	\end{tabular}
	~
	\caption{#1}\label{#2}
        \vspace{-5pt}        
\end{figure}
}

\newcommand{\myfigtwovert}[8]
{
\begin{figure}
        \centering
         \begin{tabular}{c}
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#1}
                \caption{#2}
                \label{#3}
        \end{subfigure}%
        \\
	\\
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#4}
                \caption{#5}
                \label{#6}
        \end{subfigure}
        \end{tabular}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \caption{#7}\label{#8}
        \vspace{-10pt}        
\end{figure}
}

\newcommand{\mysubfigtwovert}[8]
{
\begin{figure}
        %\centering
         \begin{tabular}{c}
        \begin{subfigure}[b]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#1}
                \caption{#2}
                \label{#3}
        \end{subfigure}%
        \\
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{#4}
                \caption{#5}
                \label{#6}
        \end{subfigure}
        \end{tabular}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \caption{#7}\label{#8}
        \vspace{-10pt}        
\end{figure}
}

\newcommand{\mysubfigthree}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\mysubfigthreecont
}

\newcommand{\mysubfigthreecont}[2]
{
\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempa}
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempd}
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}
        \begin{subfigure}[b]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{\tempg}
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \caption{#1}\label{#2}
        \vspace{-5pt}
\end{figure*}
}

\newcommand{\mysubfigthreebox}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\mysubfigthreeboxcont
}

\newcommand{\mysubfigthreeboxcont}[2]
{
\begin{figure*}
        \centering
        \begin{tabular}{ccc}
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempa}}%
                }%
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempd}}%
                }%
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempg}}%
                }%
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}
        \end{tabular}
        \caption{#1}\label{#2}
        \vspace{-10pt}
\end{figure*}
}

\newcommand{\mysubfigfourbox}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\mysubfigfourboxcont
}

\newcommand{\mysubfigfourboxcont}[5]
{
\begin{figure*}
        \centering
        \begin{tabular}{cc}
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempa}}%
                }%
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
        &
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempd}}%
                }%
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}
        \\
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempg}}%
                }%
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}
        &
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{#1}}%
                }%
                \caption{#2}
                \label{#3}
        \end{subfigure}
        \end{tabular}
        \caption{#4}\label{#5}
        \vspace{-10pt}
\end{figure*}
}

\newcommand{\mysubfigsixbox}[9]
{
\def\tempa{#1}
\def\tempb{#2}
\def\tempc{#3}
\def\tempd{#4}
\def\tempe{#5}
\def\tempf{#6}
\def\tempg{#7}
\def\temph{#8}
\def\tempi{#9}
\mysubfigsixboxcont
}

\newcommand{\mysubfigsixboxcont}[9]
{
\def\tempj{#1}
\def\tempk{#2}
\def\templ{#3}
\def\tempm{#4}
\def\tempn{#5}
\def\tempo{#6}
\def\tempp{#7}
\def\tempq{#8}
\def\tempr{#9}
\mysubfigsixboxcontcont
}

\newcommand{\mysubfigsixboxcontcont}[2]
{
\begin{figure*}
        \centering
        \begin{tabular}{ccc}
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempa}}%
                }%
                \caption{\tempb}
                \label{\tempc}
        \end{subfigure}%
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempd}}%
                }%
                \caption{\tempe}
                \label{\tempf}
        \end{subfigure}
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempg}}%
                }%
                \caption{\temph}
                \label{\tempi}
        \end{subfigure}
        \\
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempj}}%
                }%
                \caption{\tempk}
                \label{\templ}
        \end{subfigure}
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempm}}%
                }%
                \caption{\tempn}
                \label{\tempo}
        \end{subfigure}
        &
        \begin{subfigure}[b]{0.32\textwidth}
                \centering
                {%
                \setlength{\fboxsep}{0pt}%
                \setlength{\fboxrule}{1pt}%
                \fbox{\includegraphics[width=\textwidth]{\tempp}}%
                }%
                \caption{\tempq}
                \label{\tempr}
        \end{subfigure}
        \end{tabular}
        \vspace{-8pt}
        \caption{#1}\label{#2}
%        \vspace{-10pt}
\end{figure*}
}

\newcommand{\BA}{{\em begin\_atomic}}
\newcommand{\EA}{{\em end\_atomic}}
%\newcommand{\BAs}{{\em begin\_atomics}}
%\newcommand{\EAs}{{\em end\_atomics}}

\newcounter{claimcounter}[section]
\newtheorem{claim}{\sc Claim:}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}
\newcommand{\scbf}[1]{\vspace {0.05in}\noindent{\textbf{#1.}}}

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}
\newcommand{\algorithmiccontinue}{\textbf{continue}}
\newcommand{\Continue}{\State \algorithmiccontinue}

\algrenewcomment[1]{\(\triangleright\) #1}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


==> senx-discussion.tex <==
\section{Discussion} \label{sec:senx_discussion}
%- concern on the safety of the patch regarding the correctness of the predicate
\scbf{Limitations}	%A keen reader may have the impression that the symbolic expressions generated by Senx are dependent on the program path that is executed as a result of the malicious input used in the concolic execution of the target program, and hence concerns that two problematic situations might arise. First, a false negative can happen when the symbolic expressions are incorrect for a variant of the malicious input that can trigger the same buffer overflow on a different program path, in which case the patch can fail to prevent the buffer overflow triggered by the variant. Second, a false positive can happen when the symbolic expressions are incorrect for a benign input that leads to a different program path such that the patch can mistakenly reject benign inputs.

%- limitation of access range analysis
%- limitation of symbolic expression translation



==> senx-motivation.tex <==
\if 0
\lstdefinestyle{C}{
        xleftmargin=10pt,
        xrightmargin=0pt,
        basicstyle=\scriptsize\bfseries\ttfamily,
        showspaces=false,
        showtabs=false,
        breaklines=true,
        showstringspaces=false,
        breakatwhitespace=true,
        commentstyle=\color{mygreen},
        keywordstyle=\color{myblue},
        stringstyle=\color{myred},
        numbers=left,
        numbersep=5pt,
        numberstyle=\scriptsize\color{mygray},
        tabsize=2,
        frame=TB,
        framesep=5pt,
        escapeinside={\%*}{*},
        title=\lstname
        %  moredelim=[il][\textcolor{pgrey}]{$$},
        %  moredelim=[is][\textcolor{pgrey}]{\%\%}{\%\%}
}
\fi

\section{Motivation}

\subsection{Automated Patch Generation for Buffer Overflow Vulnerabilities}
% buffer overflow vulnerabiilties are still prevalent
Buffer overflow vulnerabilities is one of the earliest type of security vulnerabilities and there is a long history of research proposals that aim to tackle them \cite{stackguard}. Unfortunately they are still one of the most prevalent vulnerabilities in the wild \cite{}.

% state-of-art proposals to generate patches automatically are of low applicability and quality, and thus buffer overflow vulnerabilities continue to be patched manually
Despite a great deal of research on automating the construction of patches \cite{PAR, GenProg, DirectFix, SemFix, Angelix, SPR, CodePhage}, security vulnerabilities including buffer overflow vulnerabilities continue to be constructed manually by developers, due to the low applicability and quality of patches generated automatically \cite{}.

One critical reason for the low quality of current automated patch generation (APR) approaches is that they are agnostic to the type of bugs that they aim to patch, and thus have to rely on the result of running test suites to determine whether patches are correct or not. However, passing test suites is often insufficient to guarantee the correctness of patches \cite{}.

In light of that, we argue that APR should rely on more robust approaches rather than passing test scripts to guarantee its correctness. Our insight is to synthesize bug-specific patches by leveraging the information pertain to the type of bugs, as this methodology has been proven to be successful to fix concurrency bugs \cite{AFix, CFix}. 

To design a bug-specific APR for buffer overflow vulnerabilities, we first conduct a study on human-written patches for real-world buffer overflow vulnerabilities to understand how these vulnerabilities are fixed in practice. From the study, we aim to create a patch template and the list of the essential ingredients needed for the template, and more importantly find an effective approach to extract the ingredients for a particular buffer overflow vulnerability. With the patch template, our APR extracts needed ingredients, synthesizes a patch, and inserts the patch at an appropriate location in a program, in order to fix a particular vulnerability.

\if0
We use a typical human developer generated patch for a buffer overflow vulnerability in listing \ref{lst:simple_patch} to illustrate a template for automated patch generation for buffer overflow vulnerabilities. As we can see, the patch adds code to return to error when an out-of-bounds memory write is to be executed. The patch consists of a check on a predicate at line 7 and a control transfer statement at line 8. The predicate indicates whether the pointer \textit{p} that is used to write to a buffer starting at \textit{output} is beyond the upper bound of the buffer \textit{output + output\_size}, which is the starting address plus the size of the buffer.

\begin{lstlisting}  [float,floatplacement=T,label=lst:simple_patch,language=C,style=C,caption=A typical patch for buffer overflow vulnerability\vspace{-18pt}]
int copy_input(char *input, int input_size, char *output, int output_size) {
	char *p, *q;

	p = output;
	q = input;
	while (q < input + input_size) {
+		if (p >= output + output_size)
+			return -1;
		*p++ = *q++;
	}
	return 0;
}
\end{lstlisting}

\fi

\subsection{A Study on Real-World Buffer Overflow Vulnerabilities}\label{sec:study_vulnerabilities}
%\subsubsection{Methodology}
%To identify typical templates of human-written patches for buffer overflow vulnerabilities, for the purpose of automatically generating such kind of patches, we conducted a study on the patches for recent buffer overflow vulnerabilities. 

Our study focuses on recent buffer overflow vulnerabilities in a variety of popular and mature applications. We collect our data set from popular CVE databases. In total, our data set include \textbf{XX} buffer overflow vulnerabilities from year \textbf{XXXX} to \textbf{XXXX} for X applications as shown in table \ref{tbl:apps}.

\begin{table}
        \begin{center}
                \caption{Real World Buffer Overflow Vulnerabilities}
                \begin{tabular}{|l|l|r|r|}
                        \hline
                        \textbf{App.} & \textbf{Type} & \textbf{Vulns.} & \textbf{SLOC} \\
                        \hline
			gimp & Graphics & & \\
			libav & Video/Audio & & \\
			Linux kernel & OS & & \\
			PHP & Interpreter & & \\
			qemu & Emulator & & \\
                        \hline
		\end{tabular}
		\label{tbl:apps}
	\end{center}
\end{table}


To facilitate the collecting of patches, we wrote a web crawler that automatically crawls CVE databases for vulnerabilities whose descriptions including the keyword ``buffer overflow'', ``heap overflow'' or ``stack overflow''. For each identified buffer overflow vulnerability, the crawler follows the reference links on the description page for the vulnerability to download matching patches. Because the reference links of a vulnerability often include not just URLs to patches, we identify patches by looking for ``git:'' in a URL.

%\subsubsection{Common Models of Buffer Overflow Patches}
From the \textbf{XX} buffer overflow patches that we studied, we categorize them into five different types based on whether the patches affect the allocation or the access of a buffer, and the nature of the logic that they added or modified. 
\begin{table}
\caption{Types of Buffer Overflow Patches}
\begin{tabular}{|l|p{2.5cm}|p{3cm}|r|}
\hline
\textbf{Type} & \textbf{Description} & \textbf{Example} & \textbf{Count} \\ \hline
AC & Add a check before buffer access & if (out\_of\_bounds) {return error;}  & 10  \\ \hline
CS & Change the scope of access & memmove(d,s,c) $\Rightarrow$ memmove(d,s,4) & 3 \\ \hline
CF & Use a safe memory access method & strncpy(d,s,c) $\Rightarrow$ strlcpy(d,s,c) & 2 \\ \hline
NS & Specify the buffer size using a variable rather than a constant & p = malloc(80) $\Rightarrow$ p = malloc(c); & 2 \\ \hline
SD & Use dynamic memory allocation rather than static memory allocation & char buf[80] $\Rightarrow$ buf = malloc(count); & 3 \\ \hline
\end{tabular}
\label{tbl:type_patches}
\end{table}

Table \ref{tbl:type_patches} summarizes the five most common patch types. Column ``Type'' shows the acronym of each patch type. Column ``Description'' shows a brief description for each patch type. Column ``Example'' presents a simplified example patch. Column ``Count'' gives the number of patches belong to each patch type, for the vulnerabilities.

As we can see, type-AC is the most common type of buffer overflow patches. In this paper, we focus on type-AC patch as it fixes the most number of buffer overflow vulnerabilities in practice.

By generalizing type-AC patch, we create a template as in listing \ref{lst:patch_template}, where \textit{access\_pointer} is the pointer that accesses a buffer, \textit{error} is an error return code, \textit{buffer\_lower\_bound} and \textit{buffer\_upper\_bound} are the lower bound and upper bound of the buffer, respectively.

\begin{lstlisting}  [float,floatplacement=t,label=lst:patch_template,language=c,style=c,caption=an apr template for buffer overflow Vulnerabilities \vspace{-18pt}]
if (access_pointer < buffer_lower_bound || access_pointer > buffer_upper_bound)
	return error_code;
\end{lstlisting}

To synthesize a patch, we need to extract the ingredients including the access\_pointer, buffer\_lower\_bound, buffer\_upper\_bound, and error\_code from the program that we aim to patch. We also need to find an appropriate location to insert the patch. Note that the two needs are dependent on each other, because the ingredients must also be accessible in the scope of the location where a patch is to be inserted.

There can be more than one possible locations to insert a patch. In our current design, we always insert a patch immediately before the location where a buffer is accessed.

All the ingredients except the error\_code are dependent on the particular vulnerability. Usually human-written patches simply use an existing error\_code already present in the code, rather than add a new error\_code for the vulnerability. We identify existing error\_code in a program using an approach based on the one proposed by Talos \cite{Talos}.

To figure out how to extract ingredients that are dependent on a particular vulnerability, we conducted manual analysis on vulnerabilities that are fixed with type-AC patches, which we call type-AC vulnerabilities. 

And we categorize type-AC vulnerabilities into two kinds: \textit{simple vulnerabilities}, for which it is trivial to automatically extract the ingredients from a same function, and \textit{complex vulnerabilities}, for which it is non-trivial to automatically extract the ingredients for the following challenges.

\begin{itemize}
\item Inaccessible ingredients - For example, buffer allocation and buffer access occur in different functions where the buffer size is not directly passed from or accessible from the function where buffer is accessed.
\item Multiple sets of ingredients - For example, there exist more than execution paths on each of which the same buffer is accessed but a different set of variables are used for the access.
\end{itemize}

From our manual analysis on type-AC vulnerabilities, we find that 35\% of them are complex vulnerabilities. 

\begin{lstlisting}  [float,floatplacement=T,label=lst:example_vulnerability,language=C,style=C,caption=A complex buffer overflow vulnerability\vspace{-18pt}]
static int dpcm_decode_frame(AVCodecContext *avctx, void *data, ..., AVPacket *avpket) {
	int buf_size = avpkt->size;
	DPCMContext *s = avctx->priv_data;
	AVFrame *frame = data;
	int out = 0, ret;
	int ch = 0;
	int stereo = avctx->channels - 1;
	int16_t *output_samples, *samples_end;

    	/* calculate output size */
    	switch(avctx->codec->id) {
    	case AV_CODEC_ID_ROQ_DPCM:
        	out = buf_size - 8;
        	break;
    	case AV_CODEC_ID_SOL_DPCM:
        	if (avctx->codec_tag != 3)
            		out = buf_size * 2;
        	else
            		out = buf_size;
        	break;
    	}

    	/* get output buffer */
    	frame->nb_samples = out / avctx->channels;
        if ((ret = ff_get_buffer(avctx, frame, 0)) < 0) {
        	av_log(avctx, AV_LOG_ERROR, "get_buffer() failed\n");
        	return ret;
        }
    	output_samples = (int16_t *)frame->data[0];
    	samples_end = output_samples + out;

    	switch(avctx->codec->id) {
    	case AV_CODEC_ID_ROQ_DPCM:
	        /* decode the samples */
        	while (output_samples < samples_end) {
            		*output_samples++ = predictor[ch];
        	}
        	break;
    	case AV_CODEC_ID_SOL_DPCM:
        	if (avctx->codec_tag != 3) {
            		uint8_t *output_samples_u8 = frame->data[0],
                    	*samples_end_u8 = output_samples_u8 + out;
            		while (output_samples_u8 < samples_end_u8) {
                		*output_samples_u8++ = s->sample[stereo];
            		}
        	} else {
            		while (output_samples < samples_end) {
                		*output_samples_u8++ = s->sample[stereo];
			}
		}
		break;
	}
	return buf_size;
}
\end{lstlisting}
- Challenges in automatically constructing a patch for complex buffer overflow vulnerability




==> senx-vul_tab.tex <==
\textcolor{red}{sqlite-CVE-2013-7443} & \textcircled{3} & Determinate & \NA & \textcolor{red}{Failed} & \NA & \ding{55} \\
sqlite-CVE-2017-13685 & \textcircled{3} & Determinate & \NA & Trivial & Simple & \ding{51} \\
\hline
zziplib-CVE-2017-5976 & \textcircled{1} & Determinate & Cloned & Translated & Complex & \ding{51} \\
zziplib-CVE-2017-5974 & \textcircled{3} & Determinate & \NA & Translated & Complex & \ding{51} \\
zziplib-CVE-2017-5975 & \textcircled{3} & Determinate & \NA & Translated & Complex & \ding{51} \\
\hline
Potrace-CVE-2013-7437 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
\hline
libming-CVE-2016-9264 & \textcircled{3} & Determinate & \NA & Trivial & Simple & \ding{51} \\
\hline
\textcolor{red}{libtiff-CVE-2016-9273} & \textcircled{1} & \textcolor{red}{Indeterminate} & \NA & \NA & \NA & \ding{55} \\
libtiff-CVE-2016-9532 & \textcircled{1} & Determinate & Cloned & Trivial & Complex & \ding{51} \\
libtiff-CVE-2017-5225 & \textcircled{1} & Determinate & ARA & Trivial & Simple & \ding{51} \\
libtiff-CVE-2016-10272 & \textcircled{1} & Determinate & ARA & Translated & Simple & \ding{51} \\
libtiff-CVE-2016-10092 & \textcircled{3} & Determinate & \NA & Translated & Simple & \ding{51} \\
libtiff-CVE-2016-5102 & \textcircled{3} & Determinate & \NA & Trivial & Simple & \ding{51} \\
libtiff-CVE-2006-2025 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
\hline
libarchive-CVE-2016-5844 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
\hline
jasper-CVE-2016-9387 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
jasper-CVE-2016-9557 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
jasper-CVE-2017-5501 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
\hline
ytnef-CVE-2017-9471 & \textcircled{1} & Determinate & Cloned & Trivial & Simple & \ding{51} \\
ytnef-CVE-2017-9472 & \textcircled{1} & Determinate & Cloned & Trivial & Simple & \ding{51} \\
\textcolor{red}{ytnef-CVE-2017-9474} & \textcircled{1} & Determinate & \textcolor{red}{Failed} & \NA & \NA & \ding{55} \\
\hline
php-CVE-2011-1938 & \textcircled{1} & Determinate & ARA & Translated & Simple & \ding{51} \\
php-CVE-2014-3670 & \textcircled{1} & Determinate & ARA & Translated & Complex & \ding{51} \\
php-CVE-2014-8626 & \textcircled{1} & Determinate & Cloned & Trivial & Simple & \ding{51} \\
\hline
binutils-CVE-2017-15020 & \textcircled{1} & Determinate & ARA & Translated & Simple & \ding{51} \\
binutils-CVE-2017-9747 & \textcircled{1} & Determinate & Cloned & Translated & Simple & \ding{51} \\
binutils-CVE-2017-12799 & \textcircled{3} & Determinate & \NA & Trivial & Simple & \ding{51} \\
\textcolor{red}{binutils-CVE-2017-6965} & \textcircled{3} & Determinate & \NA & \textcolor{red}{Failed} & \NA & \ding{55} \\
binutils-CVE-2017-9752 & \textcircled{3} & Determinate & \NA & Translated & Simple & \ding{51} \\
\textcolor{red}{binutils-CVE-2017-14745} & \textcircled{2} & Determinate & \NA & \textcolor{red}{Failed} & \NA & \ding{55} \\
\hline
\textcolor{red}{autotrace-CVE-2017-9151} & \textcircled{1} & \textcolor{red}{Indeterminate} & \NA & \NA & \NA & \ding{55} \\
\textcolor{red}{autotrace-CVE-2017-9153} & \textcircled{1} & \textcolor{red}{Indeterminate} & \NA & \NA & \NA & \ding{55} \\
autotrace-CVE-2017-9156 & \textcircled{1} & Determinate & ARA & Trivial & Simple & \ding{51} \\
autotrace-CVE-2017-9157 & \textcircled{1} & Determinate & ARA & Trivial & Simple & \ding{51} \\
\textcolor{red}{autotrace-CVE-2017-9168} & \textcircled{1} & Determinate & \textcolor{red}{Failed} & \NA & \NA & \ding{55} \\
\textcolor{red}{autotrace-CVE-2017-9191} & \textcircled{1} & Determinate & ARA & \textcolor{red}{Failed} & \NA & \ding{55} \\
autotrace-CVE-2017-9161 & \textcircled{2} & Determinate & \NA & Trivial & Simple & \ding{51} \\
autotrace-CVE-2017-9183 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
autotrace-CVE-2017-9197 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
autotrace-CVE-2017-9198 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
autotrace-CVE-2017-9199 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
autotrace-CVE-2017-9200 & \textcircled{2} & Determinate & \NA & Trivial & Complex & \ding{51} \\
\hline

